EcoNAS: Finding Proxies for Economical Neural Architecture Search

Neural Architecture Search (NAS) achieves significant progress in many computer vision tasks. While many methods have been proposed to improve the efficiency of NAS, the search progress is still laborious because training and evaluating plausible architectures over large search space is time-consuming. Assessing network candidates under a proxy (i.e., computationally reduced setting) thus becomes inevitable. In this paper, we observe that most existing proxies exhibit different behaviors in maintaining the rank consistency among network candidates. In particular, some proxies can be more reliable -- the rank of candidates does not differ much comparing their reduced setting performance and final performance. In this paper, we systematically investigate some widely adopted reduction factors and report our observations. Inspired by these observations, we present a reliable proxy and further formulate a hierarchical proxy strategy. The strategy spends more computations on candidate networks that are potentially more accurate, while discards unpromising ones in early stage with a fast proxy. This leads to an economical evolutionary-based NAS (EcoNAS), which achieves an impressive 400x search time reduction in comparison to the evolutionary-based state of the art (8 vs. 3150 GPU days). Some new proxies led by our observations can also be applied to accelerate other NAS methods while still able to discover good candidate networks with performance matching those found by previous proxy strategies.

==> sections/methods-origin.tex <==
% !TEX root = ../main.tex
\section{Setup of Models and Reduced Settings}

In this section, we will introduce the experimental setups for investigating the effectiveness of the reduced settings. %for evaluating the performance of network architecture.generate the model zoo. The relative ranking change of performances for models in the model zoo will be used to evaluate the ability of different reduction factors. Then we will show how we will express the reduction factors in the following content.

\subsection{Construction of model zoo}

Each network architecture in our model zoo is the repeated stacking of two kinds of cells, normal cells and reduction cells. The model zoo contains 57 networks. The general network structure is shown in Fig.~\ref{fig:arch}(a) and we set the stack number $N=6$. The cells are generated basically following the pipeline of cell construction which is common for architecture search \cite{TNAS, ENAS, PNAS} and we just replace the search algorithm in these approaches by random sampling. Fig.~\ref{fig:arch}(c) shows the basic structure for the cells and we will provide the construction details in the supplementary material. 

\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{images/network_arch.pdf}
    \vskip -0.15cm
    \caption{Network structure overview. (a) The cell stacking method for the whole network ($N=6$). (b) The connection between cells. (c) The general cell structure, where nodes 0, 1 are input nodes. (d) The construction of nodes 2, 3, 4 in the cell. }
    \label{fig:arch}
    \vskip -0.5cm
\end{figure}

\subsection{Choice of reduction factors}
A \textbf{reduced setting} corresponds to a setting of four factors. In this paper, these factors are number of channels for CNNs ($c$), resolution of input images ($r$), training epochs ($e$), and sample ratio $s$. %These factors do not influence the architecture of a network. Therefore, the same architecture can be learned and evaluated in different reduced settings.
The value of $c$, $r$ and $s$ will be represented by a subscript $0, 1, 2, 3, 4$. The specific value for the subscript of each reduction factor for CIFAR-10 dataset \cite{CIFAR10} is shown in table \ref{tab:red_cifar10}. The subscript for $e$ will be the real value, for instance, $e_{30}$ means the number of training epochs is 30. The value of $c$ refers to the number of channels in the initial convolutional cell. %Since the channels will grow by specific multiplier at specific layers in the networks, once the initial number of channels is fixed, the channels for all layers in the networks are also determined. 
As for the sample ratio $s$, we randomly select a subset according to the value of $s$ before training and then train on this subset. Different networks are trained by different subsets, but a network is trained using the same subset during all the training epochs. For CIFAR-10, $(c_0, r_0, s_0, e_{600})$ corresponds to the original setting (also called Ground-Truth setting in the following text) used in \cite{DARTS}, which has 36 initial channels, $32\times 32$ input image, use of all samples, and trained by $600$ epochs. 
In comparison, $(c_a, r_b, s_c, e_{x})$ corresponds to a reduced setting requiring around $1/2^{a+b+c}$ FLOPs required, i.e. $2^{a+b+c}$ speed-up, when compared with $(c_0, r_0, s_0, e_{x})$. 
%Instead, we will randomly generate a new subset at each epoch, which ensures that after enough iterations, the networks can also \textit{see} all the training data. 

\begin{table}
\small
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Reduction factor & 0 & 1 & 2 & 3 & 4 \\
\hline\hline
$c$ & 36 & 24 & 18 & 12 & 8 \\
$r$ & 32 & 24 & 16 & 12 & 8 \\
$s$ & 1.0 & 0.5 & & & \\
$e$ & 30 & 60 & 90 & 120 & \\
\hline
\end{tabular}
\end{center}
\caption{Specific values of reduction factors for CIFAR-10. For the values of $c_x$ and $r_x$, if $\frac{c_0(r_0)}{({1/\sqrt{2}})^x}$ ($x$ referring to the subscript) is an integer, the integer is taken directly(such as $c_2, r_2$). If not, then the nearest number divisible by 4 is selected.}
\vskip -0.3cm
\label{tab:red_cifar10}
\end{table}

\section{Evaluation Metric for Reduced Settings}

We use Spearman Coefficient, denoted as $\rho_{sp}$, as the metric to evaluate the ability of reduced settings. It is also mentioned in \cite{PNAS} but is used to evaluate the performance of accuracy predictors. In our work, we use it to measure the dependence between the rankings of networks in the whole model zoo when evaluated in the Ground-Truth setting and the reduced setting. Eq.~\ref{eq_sp} shows the formulation of $\rho_{sp}$:

\begin{equation}
\rho_{sp} = 1-\frac{6\sum_{i=1}^{K}d_i^2}{K(K^2-1)},
\label{eq_sp}
\end{equation}

where $d_i$ is the difference for network $i$ between its ranking in the Ground-Truth setting and the new ranking in reduced setting. $K$ is the number of networks in the model zoo. 

Fig.~\ref{Fig2.sub.1}, \ref{Fig2.sub.2} show two different reduced settings with small $\rho_{sp}$ and large $\rho_{sp}$. When $\rho_{sp}$ is larger, we can see the increasing dependence of rankings between Ground-Truth setting and reduced setting for the same model.
When $\rho_{sp}$ is small, a model with low ranking at the Ground-Truth setting could have high ranking at the reduced setting frequently. In this case, the ranking for this model obtained from reduced setting becomes less reliable. Conversely, when the $\rho_{sp}$ is large, the average change of rankings from the reduced setting to the Ground-Truth is small. Therefore, higher Spearman coefficient corresponds to a more reliable reduced setting, where a good model is more likely to still be good in the Ground-Truth setting.

\begin{figure}[t]
%\begin{center}
\subfigure[Small $\rho_{sp}$]{
\label{Fig2.sub.1}
\includegraphics[width=0.23\textwidth]{images/sp_vis/72.pdf}}
\subfigure[Large $\rho_{sp}$]{
\label{Fig2.sub.2}
\includegraphics[width=0.23\textwidth]{images/sp_vis/92.pdf}}
%\end{center}
\label{fig:sp_vis}
\vskip -0.15cm
\caption{Visualization of small $\rho_{sp}$ (a) and large $\rho_{sp}$ (b). The $x$, $y$ coordinates of each point in the figure represent the rankings of a certain model in the Ground-Truth and reduced setting, respectively. For instance, point (31,10) means that the ranking of that model is 31 in the Ground-Truth setting but increases to 10 in the reduced setting.}
\vskip -0.5cm
\end{figure}

\section{Experimental Results on CIFAR-10}
\label{Sec:ExpCIFAR}
\subsection{Experimental setup}

In the Ground-Truth setting, each network in the model zoo is trained from scratch for 600 epochs with batch size 96 and the learning rate follows the cosine schedule. The setup for the reduced settings are basically the same as that for Ground-Truth setting, except for some differences, e.g. training epochs. We will list other hyper-parameters and detailed training strategies for both the Ground-Truth and reduced settings in the supplementary material.

\subsection{Analysis on effects of reduction factors}

%In this part we will comprehensively analyze the influence exerted on the network evaluation ability by the reduction dimensions, $[c,r,s,e]$.

\subsubsection{Combination of dimension $s$ and $e$}
\label{se_section}

In this part we will analyze the influence of \textbf{sample ratio} ($\textbf{s}$) and \textbf{training epoch} ($\textbf{e}$). %These two factors mainly save the total number of iterations. 
We find that training for more epochs will bring advantages but it is not a good choice to use part of the training dataset.

As shown in Fig.~\ref{Figes.sub.1}, Spearman coefficient $\rho_{sp}$ increases when increasing the number of epochs and sample ratio. Therefore, the evaluation ability improves with more training epochs and/or more training samples.  The increase of $\rho_{sp}$ from 30 epochs to 60 epochs is the most obvious, after which the profits brought by more epochs are gradually decreasing. Consider the reduced setting pairs, $c_xr_ys_0e_z$ and $c_xr_ys_1e_{2z}$ , which have the same number of iterations but $c_xr_ys_0e_z$ has fewer epochs while $c_xr_ys_1e_{2z}$ have fewer samples. By comparing  $c_xr_ys_0e_z$ and $c_xr_ys_1e_{2z} (x,y\in\{0,1,2,3,4\},z\in\{30,60\})$, we can see that training with less epochs but using the total dataset in each epoch is a better choice, especially when training for more iterations. For the same number of epochs, reducing the number of samples from 1 to 0.5 leads to obvious drop of $\rho_{sp}$. Therefore, we consider reducing sample ratio as unreliable and keep sample ratio to be 1 if not specified.
Considering the trade-off between computation consumption and profits, $s_{0}e_{60}$ will be a good combination.

We also use another metric, Hard Rank Error (abbreviated as $HRE$) to verify the robustness of our evaluation metric. The concept of HRE is also mentioned in \cite{NAO}, where it is called pairwise accuracy and we make some modifications. Opposite from $\rho_{sp}$, smaller $HRE$ indicates a better reduced setting. The detailed information and more results for $HRE$ will be provided in the supplementary material. %From Fig.~\ref{Figes.sub.2}, we can also see the similar change for more epochs and fewer samples, which means that our main metric $\rho_{sp}$ is very robust for reduced setting evaluation. 
%For different metrics, \ie $\rho_{sp}$ and $HRE$, the relative ranking for different sample ratio and numbers of epochs is consistent. 
From Fig.~\ref{Figes.sub.2}, we can see that for different metrics, the evaluation ability change for different sample ratio and numbers of epochs is consistent. This also validates that $\rho_{sp}$ is an acceptable measure for the evaluation ability of reduced settings.

\begin{figure}[t]
%\begin{center}
\subfigure[$\rho_{sp}$]{
\label{Figes.sub.1}
\includegraphics[width=0.23\textwidth]{images/epoch_sampler_sp.pdf}}
\subfigure[$HRE$]{
\label{Figes.sub.2}
\includegraphics[width=0.23\textwidth]{images/epoch_sampler_hre.pdf}}
%\end{center}
\label{fig:es}
\vskip -0.15cm
\caption{The influence of factor $s$ and $e$. The $Y$-axis is the mean $\rho_{sp}$ in (a) and mean $HRE$ (b) for 25 different reduced settings. These settings only differ in $c$  and $r$ but have the same $s$ and $e$. The lower the better for $HRE$.}
\vskip -0.4cm
\end{figure}

\subsubsection{Combination of dimension ${c}$ and ${r}$}
\label{cr_section}

In this section, we analyze the effect of factors $\textbf{c}$ and $\textbf{r}$ with fixed $s_0e_{60}$, which is also the recommended combination in the last section. We find that it is beneficial to use a smaller $c$ but reducing $r$ will bring reversed effect.

We use a 3D-Bar chart (Fig.~\ref{fig:c_r}) to show the changes along dimension $c$ ($X$-axis) and $r$ ($Y$-axis), respectively. The $Z$-axis represents $\rho_{sp}$ for each $c_xr_y$ setting and we can also clearly compare $\rho_{sp}$ from the height of the bars.  

We also use a measurement called $entropy$ denoted by $\rho_e$ to indicate the monotonicity of $\rho_{sp}$ along a certain reduction factor dimension and the details about this measurement will be shown in the supplementary material. The $entropy$ ranges from -1 to 1. The absolute value of $entropy$ close to 1 indicates that along this dimension, the objective set has an obvious monotonous increase or decrease trend, with only few small fluctuations. On the contrary, if the absolute value of $entropy$ is relatively small, such as less than 0.5, then the monotonic increase or decrease trend along this dimension is weak.

%The $\rho_e$ is measured by the Spearman coefficient between a objective set and the base set, where the objective set can be the collection of values for each row or column and the base set is $\{1,2,3,4,5\}$. Since the true values of the inputs will be transferred to the rankings, the choice of base set will not affect the final results if it is a set of increasing numbers.

As shown by the values of $entropy$ close to the $Y$-axis in Fig.~\ref{fig:c_r}, the trend along the reduction factor $c$ is obvious. %Nearly for all the $r$ settings, the smaller $c$ is, the better the corresponding reduced setting performs, except for few points e.g. $c_2r_2$. 
Nearly for all the fixed $r$ settings, a smaller $c$ leads to a better-behaved reduced setting, except for few points e.g. $c_2r_2$. The trends along $r$ for the fixed $c$ are not so consistent, reflected by the variation of $entropy$ close to the $X$-axis in the figure. But for most of the cases, a smaller $r$ will lead to decrease of $\rho_{sp}$.

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.65\linewidth]{images/e60.pdf}
\end{center}
\vskip -0.15cm
   \caption{3D-Bar chart for redution factor $c$ and $r$. The $X$-$Y$ plane shows all the combinations of $c$ and $r$ and $Z$-axis represents the corresponding $\rho_{sp}$. We can directly compare $\rho_{sp}$ through the height of the bars. The values close to the $X$ and $Y$ axis are $entropies$ which are used to evaluate monotonic increase or decrease trend for the $\rho_{sp}$ responding to the change of $r$ or $c$.}
 \vskip -0.5cm
\label{fig:c_r}
\end{figure}

\subsubsection{Combination of dimension $c$ and $e$}

In this section, we analyze the effects of $\textbf{c}$ and $\textbf{e}$ following the same method as Section~\ref{cr_section}, where the other two factors are fixed to $r_0s_0$. From the $entropies$ close to the $X$-axis of Fig.~\ref{Fig3.sub.1}, we can see that the decrease in $c$ will bring to increase of $\rho_{sp}$ for the same number of epochs, which is consistent with the results in Fig.~\ref{fig:c_r} for the same resolution. The conclusion drawn from Fig.~\ref{Figes.sub.1} and Fig.~\ref{Figes.sub.2} that more epochs will bring higher $\rho_{sp}$ is also verified in Fig.~\ref{Fig3.sub.1}.

\subsubsection{Combination of dimension $r$ and $e$}

%The effects of $\textbf{r}$ and $\textbf{e}$ with $c_0s_0$ will be discussed in this part. 
As shown in Fig.~\ref{Fig3.sub.2}, more epochs improves $\rho_{sp}$, which also validates the results in Fig.~\ref{Figes.sub.1} and Fig.~\ref{Fig3.sub.1}. Lower resolution leads to smaller $\rho_{sp}$, which is consistent with the results in Fig.~\ref{fig:c_r}.
%the entropies at the right side indicate that in the case of a relatively large $c$ ($c_0$), reducing $r$ is not a good choice, possibly due to the mismatch between the large networks and small images.

\begin{figure}[t]
%\begin{center}
\subfigure[$c_xr_0s_0e_y$]{
\label{Fig3.sub.1}
\includegraphics[width=0.23\textwidth]{images/r0.pdf}}
\subfigure[$c_0r_xs_0e_y$]{
\label{Fig3.sub.2}
\includegraphics[width=0.23\textwidth]{images/c0.pdf}}
%\end{center}
\label{fig:ce_re}
\vskip -0.15cm
\caption{3D-Bar chart of $c_xr_0s_0e_y$ (a) and $c_0r_xs_0e_y$(b), $x\in[0,1,2,3,4],y\in[30,60,90,120]$. We also show the values of $entropy$ of each dimension close to $X$ and $Y$ axis.}
\vskip -0.5cm
\end{figure}

\subsection{Discussion}
%The results we have presented provide some important insights and in this part we will discuss some extension questions which are of the same importance.
\subsubsection{Possible reason behind the profits of smaller $c$}
From the results in Fig.~\ref{fig:c_r} and Fig.~\ref{Fig3.sub.1}, we observe that the decreasing the number of channels will lead to increase of $\rho_{sp}$, which means that more reliable setting can be achieved by using fewer channels with less computation and memory.
We investigate some possible reason behind this observation.

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{images/reasoning_c_profit.pdf}
\end{center}
\vskip -0.15cm
   \caption{The value $\rho_{sp}$ as the increase of the accuracy gap. The $X$-axis is the mean difference of accuracy for networks in the model zoo between the train and test dataset at the end of training. The difference can evaluate the degree of overfitting under different reduced settings. The $Y$-axis is the corresponding $\rho_{sp}$ for each reduced setting.}
\vskip -0.5cm
\label{fig:c_reason}
\end{figure}
%Compared with the Ground-Truth setting, the total training iterations are significantly less. Therefore, if we reduce $c$, we will get a set of smaller networks which might converge faster hence are more adaptive to the limited iterations.

%We use the difference of accuracy between training and validation set to measure the convergence of networks at different reduced settings and smaller difference indicates better convergence. In Fig.\ref{fig:c_reason}, we can see that as $c$ becomes smaller, the convergence of networks becomes better and $\rho_{sp}$ is also increasing. In summary, the reason behind the benefits of smaller $c$ is likely to be due to the enhanced convergence ability.

%In Fig.~\ref{fig:c_reason}, we show the difference of accuracy between training and validation set for different settings of factor $c$. We can see that the difference becomes smaller  as $c$ becomes smaller. This indicates that the overfitting problem is less severe as $c$ is smaller. 

With smaller $c$, the amount of parameters for the same architecture will be reduced, which can help to alleviate the overfitting problem. The results in Fig.~\ref{fig:c_reason} that smaller accuracy difference between training and testing dataset appear together with smaller $c$ validate this. We hypothesize that overfitting has adverse effect on reliability on $\rho_{sp}$. 
%Therefore, the benefit of more reliable setting of smaller $c$ might be from the stability on the testing set. 
%smaller  as $c$ becomes smaller. This indicates that the overfitting problem is less severe as $c$ is smaller. 
%the degree of overfitting is decreasing with $\rho_{sp}$ increasing.  to measure the degree of overfitting of networks at different reduced settings and smaller difference indicates lower overfitting and better generalization ability. In Fig.\ref{fig:c_reason}, we can see that as $c$ becomes smaller, the degree of overfitting is decreasing with $\rho_{sp}$ increasing. 

\subsubsection{Training with large batch size at extremely reduced settings}
\label{large_bs}

Due to the increased parallelism of GPUs, when $c$ and $r$ are excessively reduced, the reduction in training time is not as obvious as the reduction in FLOPs. For instance, compared with $c_0r_0s_0e_{30}$, the FLOPs of $c_4r_4s_0e_{30}$ is $1/256$ but the consumed GPU hours are more than $1/16$. 
At some extremely reduced settings where number of channels and resolution are very small, such as $c_4r_4s_0$, we find that when the batch size is enlarged, e.g. from 96 to 384, the required execution time for one iteration is unchanged. This gives two hints. First, this validates that the more consumed GPU hours than expected is from insufficient usage of GPU. Second, we can increase the batch size by from 96 to 384 so that the number of iteration required for each epoch is reduced by 4 times.

We also conduct some experiments to explore the influence on the evaluation ability for reduction factors $c_3r_3$ and $c_4r_4$ when training with batch size enlarged from 96 to 384. The $\rho_{sp}$ of these reduced settings with large batch size are very close to those with original batch size and the difference of $\rho_{sp}$ is less than 0.02. This finding indicates that large batch size will bring us more profits, because the training time can be further reduced while basically maintaining the evaluation ability for reduced settings. %This slight decrease is acceptable considering the training time will be compressed to $1/4$ with 4 times larger batch size. 

\subsubsection{How many networks are needed to evaluate the reduced settings?}

Too few networks will cause large fluctuations of the metric, so the ability of reduced settings cannot be well evaluated. We construct a subset $\mathcal{S}$ by uniformly sampling fewer number of networks, e.g. 10, or 20, from the original model zoo. %We use the sampled networks to evaluate the 200 reduced settings. 
Denote $\{\rho_{\mathcal{S}}\}$ and $\{\rho_{Gt}\}$, respectively, as the set of Spearman coefficients for all the reduced settings obtained from sampled networks and the whole model zoo. The size of both $\{\rho_{\mathcal{S}}\}$ and $\{\rho_{Gt}\}$ are 200. And an element in $\{\rho_{\mathcal{S}}\}$ is the Spearman coefficient of the sampled models $\mathcal{S}$ in one of the 200 reduced settings. Then we use another Spearman coefficient, denoted as $\rho_{F}$ to evaluate the dependence of $\{\rho_{\mathcal{S}}\}$ and $\{\rho_{Gt}\}$.  $\rho_{F}$ evaluates the dependence between the set $\mathcal{S}$ with fewer networks and the whole model zoo. If $\rho_{F}$ is high, we can choose $\mathcal{S}$ to measure different reduced settings, which saves the resources for finding reliable reduced settings.

To eliminate deviations, for each sampling number, we conduct the sampling process 100 times and set the average dependence as the final $\rho_F$. Fig.~\ref{fig:sample} shows the dependence change with the sampling numbers. We can see that with more networks, the evaluation will become more reliable. But if the resource is limited, 15-20 networks are also acceptable %because the increase in $\rho_F$
because the profits gained from more than 20 networks are decreasing more obviously.

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{images/sample_network.pdf}
\end{center}
\vskip -0.15cm
   \caption{The dependence of $\rho_{S}$ and $\rho_{Gt}$ with the change of sampling numbers.}
\vskip -0.5cm
\label{fig:sample}
\end{figure}

\subsubsection{Will the good models still occupy the top positions in reduced settings?}
\label{retain_good}
Both the previous metrics, $\rho_{sp}$ and $HRE$ are evaluating the overall changes of the whole model zoo, however, sometimes we are more concerned about the good models. Fig.~\ref{fig:retain} shows that as $\rho_{sp}$ increases, the number of retained good models also increases, which means that reduced settings with better evaluation ability are able to keep more good models in the top positions.

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{images/retain_models.pdf}
\end{center}
\vskip -0.3cm
   \caption{Ability to retain top models for reduced settings with different $\rho_{sp}$. If a top-10 model at the Ground-Truth setting is a top-15 or top-20 model at the reduced setting, it will be considered as a 'retained good model'. We divide the reduced settings into different groups according to their corresponding $\rho_{sp}$ and calculate the average number of retained good models for reduced settings in the same group to get the $Y$-axis.}
\vskip -0.25cm
\label{fig:retain}
\end{figure}

\subsubsection{Recommendation for reduced settings}

We analyze the acceleration ratio for FLOPs and $\rho_{sp}$ of the 200 reduced settings and provide empirical results on the good reduced settings. We divide the acceleration ratio into different groups and list the reduced settings that perform best in each group. We also compare two reduced settings in \cite{TNAS}, \cite{Amoeba} where the stack number N are set to 2. In \cite{TNAS}, the reduced setting is $c_0r_0s_0e_{20}$ and in \cite{Amoeba}, the setting is $c_1r_0s_0e_{25}$. We can see that the two reduced settings in previous literature do not work very well on network evaluation.
%. In \cite{TNAS}, the networks are trained in the setting of $c_0r_0s_0e_{20}$ with $N=2$. In \cite{Amoeba}, the reduced setting is $c_1r_0s_0e_{25}$ and $N=2$. We can see that the two reduced settings in previous works do not work very well on network evaluation.}

From Fig.~\ref{fig:recomm}, we can see that many recommended reduced settings include $c_4$,  $e_{90}$, $e_{120}$. These results also verify our previous conclusions about the benefits of more epochs and less channels. 

We need to emphasize that a setting that reduces the calculation amount a lot does not necessarily have a poor evaluation ability. There are many good reduced settings that possess large acceleration ratio and outstanding evaluation ability at the same time, just as the orange points in Fig.~\ref{fig:recomm}.

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{images/recomm.pdf}
\end{center}
\vskip -0.15cm
   \caption{$\rho_{sp}$ as the acceleration ratio for FLOPs. The $X$-axis represents the ratio of FLOPs at the Ground-Truth setting to FLOPs at the reduced setting. The $Y$-axis is the $\rho_{sp}$. Along the $X$-axis, the reduced settings are getting faster and along the $Y$-axis getting better. The blue points are all the reduced settings and the orange points are recommended ones.}
\vskip -0.35cm
\label{fig:recomm}
\end{figure}


\section{Verification Experiments on ImageNet}

Due to the limited computation resources, we do not conduct comprehensive experiments on ImageNet, but only make some verification.

We randomly choose 15 architectures from the model zoo and use them to evaluate the reduced settings on ImageNet. Different from the structures for CIFAR-10, we set stack number $N=4$ and enlarge $c_0$ to 48. The training details of Ground-Truth and reduced settings will be provided in the supplementary material. The choice of reduction factors for ImageNet are shown in table~\ref{tab:imnet_red} and considering the worse effects brought by $s$, we only investigate the effects of $c$, $r$ and $e$. 

The $\rho_{sp}$ of different reduced settings are shown in Fig.~\ref{fig:imnet}. From $c_0r_0e_{10}$ to $c_0r_0e_{40}$, we can see the profits brought by more epochs but the increment of $\rho_{sp}$ also decreases. Considering the profits and time consumption,
$e_{30}$ would be a good choice. The experiment results also indicate that $c_1r_1e_{30}$ and $c_2r_2e_{30}$ are also good reduced settings for network evaluation on ImageNet. However, the setting $c_3r_3e_{30}$ performs very bad, probably due to that too small networks and resolution cannot adapt to the large dataset.

\begin{table}
\small
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Reduction factor & 0 & 1 & 2 & 3\\
\hline\hline
$c$ & 48 & 32 & 24 &  16 \\
$r$ & 224(256) & 168(192) & 112(128) & 84(96) \\
$e$ & 10 & 20 & 30 & 40 \\
\hline
\end{tabular}
\end{center}
\vskip -0.15cm
\caption{Reduction Factors for ImageNet, the values in the bracket at $r$ column refer to the resized resolution for test datasets.}
\vskip -0.2cm
\label{tab:imnet_red}
\end{table}

\begin{figure}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=0.8\linewidth]{images/imagenet_results.pdf}
\end{center}
\vskip -0.15cm
   \caption{$\rho_{sp}$ for reduced settings on ImageNet}
\vskip -0.5cm
\label{fig:imnet}
\end{figure}

